Duolando: Follower GPT with Off-Policy Reinforcement Learning for Dance Accompaniment

We introduce a novel task within the field of 3D dance generation, termed dance accompaniment, which necessitates the generation of responsive movements from a dance partner, the "follower", synchronized with the lead dancer's movements and the underlying musical rhythm. Unlike existing solo or group dance generation tasks, a duet dance scenario entails a heightened degree of interaction between the two participants, requiring delicate coordination in both pose and position. To support this task, we first build a large-scale and diverse duet interactive dance dataset, DD100, by recording about 117 minutes of professional dancers' performances. To address the challenges inherent in this task, we propose a GPT-based model, Duolando, which autoregressively predicts the subsequent tokenized motion conditioned on the coordinated information of the music, the leader's and the follower's movements. To further enhance the GPT's capabilities of generating stable results on unseen conditions (music and leader motions), we devise an off-policy reinforcement learning strategy that allows the model to explore viable trajectories from out-of-distribution samplings, guided by human-defined rewards. Based on the collected dataset and proposed method, we establish a benchmark with several carefully designed metrics.

==> content/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes See Supplementary file.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA
	\item Did you include complete proofs of all theoretical results?
    \answerNA
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes \textcolor{blue}{But the current github link is in private state. We wish make it public after fully cleaning and reformulating. The release is expected to be no later than the conference.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes
  \item Did you mention the license of the assets?
    \answerYes
  \item Did you include any new assets either in the supplemental material or as a URL?
   \answerYes
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes In datasheet.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes See supplementary file.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA \textcolor{blue}{All released data do not include personal/detectable information (like face) of the dancers. The recording process did not involve any potential harmful issue to the dancers.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes The user study participants received ice-cream vouchers as pay back.
\end{enumerate}

\end{enumerate}

==> content/sup_impact.tex <==

The task we're proposing - dance accompaniment - holds significant potential for enhancing a multitude of VR/AR applications, including the prospect of virtually dancing alongside AI. Furthermore, research into human-human interaction could substantially aid in improving the immersive and interactive experiences offered by VR games.
%
However, the research on real-looking motion generation in response to human may also lead to AI fraud, where the existing verifying methods could be more difficult to judge whether it is fake based on response.

==> tables/tab_datasets_full.tex <==
\begin{table}
    % \vspace{-3mm}
    
\caption{\small\textbf{Comparison with existing music-to-dance datasets.} HHI denotes Human-Human Interaction. Dancers means professional performers.
%
}
% \vspace{-8pt}
\centering
\footnotesize
{
\begin{tabular}{l c c c c c c m{3cm} }
\toprule

Dataset & HHI & Hands & \makecell{Ground \\ Truth} & Acquisition & \#Dancers & Hours & Genres \\ % highlight hands?
\midrule

% HMM [] \\
Dance Melody~\misscite & - & - & 3D Joints & MoCap & 13 & 1.57 & Waltz, Tango, Cha-Cha, Rumba \\
\hline
DanceNet~\misscite & - & \checkmark & 3D Joints & MoCap & 2 & 0.96 & Modern, Curtilage\\
\hline
%YT-Dance3D~\misscite & - & - & rich & MoCap & n/a & 5\\
Dancing2Music~\misscite & - & - & 2D Joints & Auto & n/a & 71 & Ballet, Zumba, Hip-Hop\\
\hline
DanceRevolusion~\misscite & - & - & 2D Joints & Auto & n/a & 12 & Ballet, Japanese Pop, Hip-Hop \\
\hline
PMSD~\misscite & - & \checkmark & 3D Joints & MoCap & 1 & 3.1 & Hip-Hop, Popping, Krumping\\
\hline
ShaderMotionVR~\misscite & - & - & 3D Joints & VR Tracker & 8 & 9 & Freestyle, Ballet\\
\hline
AIST++~\misscite & - & - & SMPL & Auto & 30 & 5.2 & 4 Old School (Break, Pop, Lock, Waack) and 6 New School (Middle Hip-Hop, LA-style Hip-hop, House, Krump, Street Jazz, Ballet Jazz)\\ % Old School (Break, Pop, Lock and Waack) and New School (Middle Hip-hop, LA-style Hip-hop, House, Krump, Street Jazz and Ballet Jazz).
\hline
PhantomDance~\misscite & - & - & SMPL & Artists & 100+ & 9.6 & Otaku Dance, Hip-hop, Jazz, Old School \\ % Otaku Dance, Hip-hop, Jazz and Old School
\hline
AIOZ-GDANCE~\misscite & - & - & SMPL & Semi-auto & 4000+ & 16.7 & n/a \\
\hline\hline
\dname & \checkmark & \checkmark & SMPL-X & MoCap & 10 & 1.92 & 5 Latin (Cha Cha, Lumba, Samba, Pasidobal, Jive), 4 Modern (Foxtrot, Tango, Quickstep, Waltz), and \textit{Pas de Deux} ballet\\

% ATD-12K \cite{siyao2021deep}  &   \textbf{302} & -- & -- & --& -- \\
% CreativeFlow+ \cite{shugrina2019creative}       & 49       &  0.82     &3.84 (11.34)$^*$   &  16.40     & 373.68 (1106.01)$^*$\\ % & 1598.32\\
% AnT \cite{casey2021animation} (private)        & < 50$^\dag$& --    &  --   & --     & --         \\
% DD100 (ours)               &  237      & \textbf{9.59}  & \textbf{19.27} & \textbf{19.09}  &  \textbf{1774.43}  \\ % & \textbf{1731.46}\\

% \midrule
% \textit{Agent 327}      &   409     & 14.06   & 14.55  & 16.14   & 1478.94  \\%   & 1582.21\\
% \textit{Caminandes 3}  &   152     & 8.17     & 24.53  & 22.39   & 2168.02  \\ %  & 2102.94\\
% \textit{Sprite Fright}  &   250     & 7.45    & 10.01  & 13.24   & 1118.86  \\ %  & 939.82\\



% Dataset &    \# Seg. & \# Occ. Seg. & Avg. Pix. shift & Avg. Seg. shift  &  Accum. Pix. shift \\ % & Seg. shift\\ 
% &  per Fr. & per Fr. & per Fr. & per Fr. & per Seq. \\%& per Seq. \\
%       \midrule
% ATD-12K \cite{siyao2021deep}  &   \textbf{302} & -- & -- & --& -- \\
% CreativeFlow+ \cite{shugrina2019creative}       & 49       &  0.82     &3.84 (11.34)$^*$   &  16.40     & 373.68 (1106.01)$^*$\\ % & 1598.32\\
% AnT \cite{casey2021animation} (private)        & < 50$^\dag$& --    &  --   & --     & --         \\
% AnimeRun (ours)               &  295      & \textbf{6.31}  & \textbf{20.09} & \textbf{19.04}  &  \textbf{2426.38}  \\ % & \textbf{1731.46}\\

% \midrule
% \textit{Agent 327}      &   420     & 9.05   & 14.55 & 17.27  & 1332.96  \\%   & 1582.21\\
% \textit{Caminandes 3}  &   166     & 6.46  & 28.10  & 24.81  & 3731.44  \\ %  & 2102.94\\
% \textit{Sprite Fright}  &   386     & 3.23  & $\,$ 7.61   & 11.51   & 621.61 

    \bottomrule
  \end{tabular}
  }
  \label{table:data_comparison}
%   \vspace{-15pt}
\end{table}
